Transfer Learning for Human Activity Recognition using Representational Analysis of Neural Networks

Human activity recognition (HAR) research has increased in recent years due to its applications in mobile health monitoring, activity recognition, and patient rehabilitation. The typical approach is training a HAR classifier offline with known users and then using the same classifier for new users. However, the accuracy for new users can be low with this approach if their activity patterns are different than those in the training data. At the same time, training from scratch for new users is not feasible for mobile applications due to the high computational cost and training time. To address this issue, we propose a HAR transfer learning framework with two components. First, a representational analysis reveals common features that can transfer across users and user-specific features that need to be customized. Using this insight, we transfer the reusable portion of the offline classifier to new users and fine-tune only the rest. Our experiments with five datasets show up to 43% accuracy improvement and 66% training time reduction when compared to the baseline without using transfer learning. Furthermore, measurements on the Nvidia Jetson Xavier-NX hardware platform reveal that the power and energy consumption decrease by 43% and 68%, respectively, while achieving the same or higher accuracy as training from scratch.

==> files/broader_impacts.tex <==
\section*{Ethics statement}
% Movement disorders are one of the leading causes of functional disability in the elderly population. 



Movement disorders, such as Parkinson's disease (PD) and essential tremor (ET) affect more than 70 million people worldwide~\cite{daneault2018could} and severely hinder their Quality-of-Life~(QoL).
Current treatment for movement disorder patients relies on visits to the clinic where a specialist observes the symptoms in a clinical environment~\cite{espay2016technology}.
However, there are no standard approaches to monitor their progress once the patient leaves the clinic.
Therefore, recent research has called for the development of devices and algorithms that enable the monitoring of activities and symptoms of patients~\cite{espay2016technology,ozanne2018wearables}.

Human activity recognition is the first step towards a solution to movement disorders as it enables continuous monitoring of patients' activities in a free-living environment. It also aids doctors with knowledge of what their patient is doing before reaching a conclusion~\cite{daneault2018could}.
However, training classifiers for movement disorder patients is challenging since there is wide variability in the severity of their symptoms, which affects the activity patterns.
The proposed approach helps in this process by enabling the transfer of general features among patients and the fine-tuning the layers that provide user-specific information.
As a result, our approach will take us one step closer to personalized healthcare for movement disorders.
Furthermore, it can potentially facilitate monitoring movement disorder symptoms, such as freezing of gait and resting tremor.

The computational savings achieved by the proposed approach can potentially aid in preserving the data privacy of users by enabling fine-tuning CNNs on the device. The on-device fine-tuning avoids the transfer of raw user data to the cloud, thus preserving the privacy of the data.
This is especially crucial for health records since any leak of the data can have serious consequences for the patients' well-being.

To the best of the authors' knowledge, this work does not disadvantage any person directly. At the same time, the authors acknowledge that any activity recognition system can potentially be used with malicious intent, such as tracking user movements. Therefore, the devices and algorithms must be sufficiently secured and encrypted such that any malicious use can be prevented.

If the HAR classifiers are directly used to make decisions for patients, potential failures in the classification would affect the users' qualify of life. Therefore, the data and insights on patient activity from HAR classifiers must be verified by health professionals before making any decisions. This information has to be disclosed to the users.
Finally, the proposed approach does not leverage any bias in the datasets used for validation. 


